A Cross-Repository Model for Predicting Popularity in GitHub

Social coding platforms, such as GitHub, can serve as natural laboratories for studying the diffusion of innovation through tracking the pattern of code adoption by programmers. This paper focuses on the problem of predicting the popularity of software repositories over time; our aim is to forecast the time series of popularity-related events (code forks and watches). In particular, we are interested in cross-repository patterns-how do events on one repository affect other repositories? Our proposed LSTM (Long Short-Term Memory) recurrent neural network integrates events across multiple active repositories, outperforming a standard ARIMA (Auto-Regressive Integrated Moving Average) time series prediction based on the single repository. The ability of the LSTM to leverage cross-repository information gives it a significant edge over standard time series forecasting.

==> sections/1_introduction.tex <==
During recent decades social networks have been the most powerful tools that enable people share information or collaborate in successful completion of project tasks such as development of software codes \cite{begel2010social,storey2010impact}. 
One of the very popular used coding platform is
GitHub. It hosts many development projects and provides a space for professionals who work together. GitHub is relatively unique compared to other social networks since developers with different backgrounds, interests  and  levels of proficiency interact with each other for asynchronous team-based software development and this provides an opportunity to investigate team-based communities evolution for researchers. Recently, there have been many studies on GitHub. Authors in \cite{vasilescu2015gender,calefato2017preliminary} investigate key drivers and behaviors in GitHub projects and teams through study social behavior and teamwork in communities on GitHub. Some others \cite{vasilescu2013stackoverflow,gousios2014exploratory,ray2014large,vasilescu2015data} investigate the impact of utilizing this platform on the software development process. Much of the work in this area employ data-driven approaches with the available data to investigate social behaviors or teamwork communication \cite{soares2018factors,aggarwal2014co,casalnuovo2015developer}. In addition to data-driven techniques, there are also several examples of survey and interview studies \cite{dabbish2012social, marlow2013impression,vasilescu2015perceptions}.

In this work we investigate network semantic segmentation with application to GitHub to segment the network into the different parts according to the topics of area such as machine learning, algorithm, game development, etc. We employ users' attributes alongside with the network connections to group the GitHub users. This type of network segmentation can reveal significant information for social network analysis regarding evolution of areas such as machine learning, algorithms, game development, etc.
 We compare three approaches for such segmentation.  First, community ensemble combines multiple communities
into a single segment. Second, user-network attributes clustering. We augment node attributes with network significant connections for network
semantic segmentation. We then employ machine learning approaches for clustering
the users. Finally, clustering approach which uses only users’ profile
attributes to classify them. Our evaluation was conducted on a
dataset composed of the public GitHub events and repository profiles from 
2015 through 2017.

The remainder of this paper is organized as follows. Section \ref{DataDescription} describes
our dataset. Section \ref{Problem-Definition} and \ref{Method} states the problem and our method respectively.  Results are provided in Section \ref{Results} and then we conclude the
paper in section \ref{conclusion}.

==> sections/2_section.tex <==
\label{DataDescription}
In this study, we consider GitHub online social networks from which we extract the communities. GitHub with having almost 20 million users and 57 million repositories is the largest host of source code in the world at the moment.\\

Before describing the data in detail, we will introduce some terms in this data set to go further.\\\\
\textbf{Definitions}: 
\begin{itemize}
    \item \textbf{Repository:}   is   a   location   where   a   particular   project and  all  files  associated  with  it  are  stored.  It  is  usually abbreviated  to  “repo”.
    \item \textbf{Event:}  refers  to  the  various  activity  streams  on  GitHub. Developers have different kind of interaction with repositories such as pulling, pushing, commiting, etc. These events are considered as the links between user nodes as repository nodes.
    \item \textbf{User:} refers to any person or organization who have created a profile on GitHub platform. 
    
    \item \textbf{Topic}: represents intended purpose, subject area, affinity groups, or other important qualities of the repository related to a project.
     \item \textbf{Community} refers to a group of users which highly interact with the same repositories by creating different types of events.
\end{itemize}


The observation period for community structure that we mined to analyze was from first January 2015 until January 2017. We decided
to select the portion of data which were of great importance and our resources let us to work with.
So we focused on Top-1000 repositories. To retrieve these two samples, we
order the repositories by their activities which we considered as the number of events corresponding to them and selected 1000 unique repositories respectively.
We have filtered those users who interact with these active repositories.
We have extracted the events corresponding to the users whose information is publicly available which were about 8437 users. From these events we then created the repository-user network.
The resulting network was a bi-partite graph with repositories in the first set and users in the second set. This network is then projected on users node to come up with users network. With the new graph we were able to capture the user communities with common community detection algorithms. Louvain algorithm is the one we applied on the latter network and the actual communities are detected by it.


The Louvain community detection algorithm is an efficient method for identifying communities in large networks. \\
  We explain the problem in section \ref{Problem-Definition} and our approach in \ref{Method} in details.


==> sections/3_section.tex <==
\section{Problem Statement}
\label{Problem-Definition}

Finding the semantic segments of network consist of groups of users with the same area of work or interest is our goal. Mathematically, we are addressing the following problem.

\textbf{Problem definition:}\\
We consider a $G=(U,V,E,C,T_{t})$ to denote a bipartite graph whose partition has the parts $U$ and $V$, and $E$ denotes the edges of the graph. Each nodes $u_{i}$ and $v_{i}$ belong to $U$ and $V$ set has $n$ and $m$ attributes and represented with ${u_{i}}_{f_{1}ft_{2},..,f_{n}}$ and  ${v_{i}}_{f_{1},f_{2},..,f_{m}}$ respectively. $C$ is a $|C| <= N$
communities associated with users. Each user belongs to a communities. Our goal is to split network semantic into $T$ segments where each of them consists of users associating with a class label  $t \in T$ representing a set of topics. Fig. 
\ref{fig:Ecosystem} shows a small scale GitHub networks. Users interact with different repositories which each repository is associated with a range of topics.
\begin{figure}[h]
\centering
	\includegraphics[height=6cm,width=10cm]{topic-clustering.png}
	\caption{Github Semantic Segmentation}
	\label{fig:Ecosystem}
\end{figure}

==> sections/4_section.tex <==
section{Method}
\label{Method}
To address the problem stated in section \ref{Problem-Definition} we propose and investigate the performance of three approaches:
\begin{itemize}
    \item \textbf{Community ensemble}: This approach combines multiple communities which have been already detected by community detection algorithms into a single segment. This approach is among the consensus solutions. We employ hierarchical agglomerative clustering (HAC) for this purpose. We have labeled each community members with the common topic among all the members. The distance of communities with the same labels would be zero. Otherwise they would be combined according to the distance between their labels. 
    
    \item \textbf{User-network attribute clustering}: This approach use the regular clustering algorithms to apply the semantic segmentation in such a way that they are similar in terms topic attribute as well as network structure. meaning that they interact with similar repositories or belong to the same community. We use the most active repositories as categorical attribute for users. 
    
    \item \textbf{Classic clustering}: This method is regular clustering approach using the users attributes to classify them.
\end{itemize}
We have followed the following steps to find the semantic segments on GitHUb:

\begin{enumerate}
    \item \textbf{Building the graph}\\

 We have created the corresponding graph using Networkx package. We used anonymized users and repo ids to fed into networkX graph as nodes. Our target graph consists of repositories and users as $U$ and $V$ sets respectively and events in our study dataset who indicate the edges of the network and represented as $E$. 


\item \textbf{Extracting network structure attribute}
The well known repositories can be a measure to categories the users. For example if some users highly interact with TensorFlow which is an open-source software library for data flow programming and broadly used in machine learning area, they can be be grouped into one category if they are close enough in terms of other attributes as well. 

\item{\textbf{Network Graph Projection}}
To detect the community of users we have used graph projection method on user-repository bipartite graph.
 Bipartite network projection is an broadly used technique for condensing information about bipartite networks. By this way two users interacting with the same repository are connecting to each other via an edge. Figure \ref{fig:Projection} represents an example to show the way we have created user graph from original bi-partite graph.


\begin{figure}[t]
\centering
	\includegraphics[height=6cm,width=8
cm]{Capture2.PNG}
	\caption{GitHub Network Projection Example}
	\label{fig:Projection}
\end{figure}




\item{\textbf{Community Detection}}
Having the user network graph, we have applied Louvain algorithm to determine the actual community that exist in the current network. Louvain method targets the modularity of the detected communities.
With this approach the quality of a community assignment is measured and quantified by the density of the connections which exist within communities compared to a particular type of random network. 
 Until here we have detected the communities which users are associated with and have labeled each user with its community label.  

\item {\textbf{One Hot Encoding}}
Those attributes that we use are categorical features. Machine learning algorithms are not able to use categorical
data directly. Also, there is no ordinal relationship between the features we have selected. Therefore, we have used one hot coding for the topic features. 

\item {\textbf{Unsupervised Clustering}}


After we extracted the network feature of target nodes and added them to the node attributes as additional ones, we then employed clustering techniques. Clustering algorithms are used to find similar groups in data as clusters. As we are taking advantage of network features alongside with other features, similarity would be measured based on both advanced features as well as the other attributes such as topic of interest. We have tried multiple clustering algorithms such as Mini Batch KMeans, MeanShift, Ward, Birch and Agglomerative Clustering. We finally selected Mini Batch KMeans and Birch for regular clustering approach and Agglomerative Clustering for community ensemble based on the precision and time complexity of these algorithms.

\begin{figure}[t]
\centering
	\includegraphics[height=5cm,width=10cm]{Agg2.jpg}
	\caption{Agglomerative approach}
	\label{fig:One-hot-encoding}
\end{figure}

\end{enumerate}



==> sections/5_section.tex <==

\section{Unsupervised Clustering}
\label{Clustering}

After we extracted the network feature of target nodes and added them to the node attributes as additional ones, we then employed clustering techniques. Clustering algorithms are used to find similar groups in data as clusters. As we are taking advantage of network features alongside with other features, similarity would be measured based on both advanced features as well as the other attributes such as topic of interest. We have tried multiple clustering algorithms such as Mini Batch KMeans, MeanShift, Ward, Birch and Agglomerative Clustering. We finally selected Mini Batch KMeans and Birch for regular clustering approach and Agglomerative Clustering for community ensemble based on the precision and time complexity of these algorithms.

\begin{enumerate}
\item Mini Batch K-Means:\\
k-means clustering aims to partition $n$ observations into $k$ clusters in which each observation belongs to the cluster with the nearest mean \cite{sculley2010web}, serving as a prototype of the cluster. This results in partitioning of the data space into Voronoi cells. Mini batch k-means reduces the computational cost of finding a partition is proportional to the size of the sample batch in comparison to K-means.\\

\item Birch:
BIRCH (balanced iterative reducing and clustering using hierarchies) is an unsupervised algorithm which clusters the multi-dimensional data in an incrementally way. This makes the BIRCH a proper clustering algorithm for large data-set. Also, in most cases, BIRCH only scan the database once. \cite{zhang1996birch}
\item Agglomerative:\\
This algorithm uses a bottom up approach \cite{steinbach2000comparison}. Pairs of clusters group into together and move up. The key operation of Agglomerative is computing the distance matrix. We labeled each cluster with the common topics vector between the communities in the cluster. Grouping the communities is based on the distance of the communities topic label vector in each step.

\begin{figure*}[t]
\centering
	\includegraphics[height=5cm,width=10cm]{Agg2.jpg}
	\caption{Agglomerative approach}
	\label{fig:One-hot-encoding}
\end{figure*}
\end{enumerate}

==> sections/6_section.tex <==
\section{Results}
\label{Results}

To evaluate the methods we have focused on the diversity of communities in the segments after using each approach. All three approaches group the users into the segments which are categorized as different topics. However, not only it is important that users be  grouped into the categories with the true label of topic, but also it is significant that they belong to the semantic segment that they have the higher number of interactions.
Diversity is the quantitative measure to reflects how many different types of communities there are in each semantic segment. 
There are multiple metrics to evaluate the diversity of members inside a semantic segment.
The Shannon index also known as Shannon's diversity index or Shannon–Wiener index has been a popular one to quantify the entropy. Shannon-Wiener diversity index is defined as:
\begin{equation}
H = - \sum_{i=1}^{s} p_{i}*ln(p_{i})
\end{equation}

where $s$ is the number of communities and $p_{i}$ is the proportion of the semantic segment represented by community $i$. We have used python skbio package providing which provides educational resources to calculate The Shannon index.

Another metric that we have considered to compare the approaches,is the total number of topics covered by each algorithm. Figures \ref{fig:entropy}-\ref{fig:net-topic-coverage} show the comparison results.






\begin{figure}[!h]
	\centering
	\begin{minipage}[t]{4cm}
	\centering
    \includegraphics[height=4cm,width=5cm]{entropy.png}
	\caption{Semantic segment entropy}
	\label{fig:entropy}
	\end{minipage}
	\hspace{3cm}
	\begin{minipage}[t]{4cm}
		\centering
\includegraphics[height=4cm,width=5cm]{Topic_coverage.png}
	\caption{Semantic segment topics coverage}
	\label{fig:topic-coverage}
	\end{minipage}
 
	\begin{minipage}[t]{4cm}
		\centering
\includegraphics[height=4cm,width=5cm]{entropy_repo_topic.png}
	\caption{Semantic segment entropy - having network structure attributes alongside with topics in clustering}
	\label{fig:net-entropy}
	\end{minipage}
	\hspace{3cm}
	\begin{minipage}[t]{4cm}
		\centering
\includegraphics[height=4cm,width=5cm]{Topiccoverage-repo-topic.png}
	\caption{Semantic segment topics coverage - having network structure attributes alongside with topics in clustering}
	\label{fig:net-topic-coverage}
	\end{minipage}
\end{figure}

As Figure \ref{fig:entropy} shows agglomerative approach has a lower diversity of entropy. Meaning that users in each segment have a higher degree of interaction. They belong to a narrower range of communities and therefore they mostly highly interact with the other users in the same segment. Birch grouped the people of wider range of communities into segments. Users of each segment have similarities in terms of topic of interest or activity however they belong to wider range of communities and have less interaction with the users of the same segment. Mini Batch K-means  captured the segments with even higher range of communities compared to the other two approaches.
On the other hand, agglomerative approach could cover fewer range of topics. This is due the fact that we use majority voting approach to label the communities and segments as the hierarchy goes up. Birch can cover a wider range of topics and Mini batch K-means covered the highest range of topics.
Having network structure as attributes alongside with topic attributes could decrease the entropy while capture more topics. Therefore, it outperforms the agglomerative algorithm in terms of topic coverage and clustering based on only topics in terms of entropy. 
%\input{referenc}

==> sections/7_conclusion.tex <==
\section{Conclusion}
\label{conclusion}
We introduced the concept of network semantic segmentation in social networks which can be very useful for these network analysis. We compared three approaches for such segmentation. First,
community ensemble combines multiple communities into a single  segment. Communities are grouped with regard to common topics among all their members. Second, user-network attribute clustering using the regular clustering algorithms to group the users into segments based on their similarity in topics as well as network attributes. It uses the most popular repositories as categorical attributes for users. 
Finally, clustering approach which uses the users' attributes to classify them.
We employed methods above on a dataset consists of 3 years GitHub data.
